Uncertainty in Contrastive Learning: On the Predictability of Downstream Performance

The superior performance of some of today's state-of-the-art deep learning models is to some extent owed to extensive (self-)supervised contrastive pretraining on large-scale datasets. In contrastive learning, the network is presented with pairs of positive (similar) and negative (dissimilar) datapoints and is trained to find an embedding vector for each datapoint, i.e., a representation, which can be further fine-tuned for various downstream tasks. In order to safely deploy these models in critical decision-making systems, it is crucial to equip them with a measure of their uncertainty or reliability. However, due to the pairwise nature of training a contrastive model, and the lack of absolute labels on the output (an abstract embedding vector), adapting conventional uncertainty estimation techniques to such models is non-trivial. In this work, we study whether the uncertainty of such a representation can be quantified for a single datapoint in a meaningful way. In other words, we explore if the downstream performance on a given datapoint is predictable, directly from its pre-trained embedding. We show that this goal can be achieved by directly estimating the distribution of the training data in the embedding space and accounting for the local consistency of the representations. Our experiments show that this notion of uncertainty for an embedding vector often strongly correlates with its downstream accuracy.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\textbf{On the marginal effect of consistency in $p^{k,\tau}_\text{emb}$.} In our experiments, consistency seems to have a very marginal (and within margin of error) effect on improving the uncertainty estimation measures. We hypothesize that such behavior could be due to a highly accurate pre-training, resulting in a high correlation between consistency and density. This correlation could be measured at larger scale and across different setups and datasets (with different accuracies) to validate this hypothesis. 

\textbf{Generalization to larger-scale datasets.} Given the assumption behind uniformity discussed by \cite{wang2020understanding}, using a GMM may be expensive on larger-scale datasets such as ImageNet \cite{imagenet}. In that case, a more sophisticated density estimation method such as a neural network, may be needed.

%In conclusion, we explored the possibility of estimating a reliability/uncertainty measure for the abstract embeddings of contrastive models in a black-box setting. We show that our uncertainty measures not only are able to meaningfully detect out-of-distribution samples but also are predictive of performance in downstream tasks.  
%We believe that having such notion of reliability/uncertainty can particularly be insightful, e.g., for deciding between different options of pre-trained models, or for deciding on specific sample weighting policies in downstream fine-tuning tasks.
